Towards causal benchmarking of bias in face analysis algorithms

Measuring algorithmic bias is crucial both to assess algorithmic fairness, and to guide the improvement of algorithms. Current methods to measure algorithmic bias in computer vision, which are based on observational datasets, are inadequate for this task because they conflate algorithmic bias with dataset bias. To address this problem we develop an experimental method for measuring algorithmic bias of face analysis algorithms, which manipulates directly the attributes of interest, e.g., gender and skin tone, in order to reveal causal links between attribute variation and performance change. Our proposed method is based on generating synthetic ``transects'' of matched sample images that are designed to differ along specific attributes while leaving other attributes constant. A crucial aspect of our approach is relying on the perception of human observers, both to guide manipulations, and to measure algorithmic bias. Besides allowing the measurement of algorithmic bias, synthetic transects have other advantages with respect to observational datasets: they sample attributes more evenly allowing for more straightforward bias analysis on minority and intersectional groups, they enable prediction of bias in new scenarios, they greatly reduce ethical and legal challenges, and they are economical and fast to obtain, helping make bias testing affordable and widely available. We validate our method by comparing it to a study that employs the traditional observational method for analyzing bias in gender classification algorithms. The two methods reach different conclusions. While the observational method reports gender and skin color biases, the experimental method reveals biases due to gender, hair length, age, and facial hair.

==> Comments__from_readers.tex <==
\section{Manmatha - 2020-05-11}

a) The approach posits that the problems with bias are not due to a lack of samples of dark people but instead due to a lack of samples of faces  with other attributes such as long hair. I think it would be more convincing if even on a small sample it can be demonstrated that augmenting and retraining a classifier according to this prescription  fixes the problem vs augmenting with images of  darker people. Otherwise, one is left to wonder which approach - real or synthetic dataset - provides the right answer. Also I wonder if by changing the distributions, it changes the overall accuracy in the real world ( since priors have a strong affect on overall  accuracy vs accuracy for sub-groups).

b) Some of the face annotations  in  Figures 6b and 9 are puzzling and make me wonder if there is an annotator bias problem. I wonder if the same annotator saw multiple images from a transect and whether this biased them to view somebody as more female or male. Or whether the annotators are all from certain ethnic backgrounds and are biased due to that. There is some literature on this and I left a citation in the feedback. 

c) The GAN conflates some attributes (eg males with longer hair get more facial hair). This is mentioned at the end. I do not know if orthogonalization eliminates this effect. If not, doesn’t this introduce a bias in the study.  Does this need to be addressed in some way?


\section{Mullainathan - 2020-05-15}
Pietro and Guha
Let me start by saying this is a much crisper draft and I really enjoyed it. 

Two points in case useful. 

Point 1
I think you have a *much* stronger case that you could lay out in abstract and your Introduction. What I say relates to a point in your original email 
b) Correlational results have no guarantee to carry over to new
situations, where the statistics of the data, and thus the
correlations, may be different. Instead, causal observations
generalize much better.

I think think you're being entirely too generous to the kinds of evaluation data that people are using. Let me give two examples: 

Case A: Suppose for a minute that the evaluation data were job applicants to a company- the correlations in *that* data at least have some meaning.  

Case B: Instead what people are actually using are data constructed using some ad hoc sampling procedures, which in turn produces a set of truly spurious correlations - they are not correlations in the wild, for some context we care about. Instead they are artificial correlations that arise from however the sample itself was constructed.  

The data in A is naturalistic and the correlations there are of a very different kind from the data in B. The correlations in B are truly spurious. And, especially in vision, the vast majority come from Case B - convenience datasets whose sampling properties are entirely unknown/arbitrary. And your striking application comes from Case B as well. 

So you have a much stronger line of attack if you say "these spurious correlations produce truly meaningless estimates of algorithmic bias."  As it stands the writing seems to (almost) imply that lots of data is in Case A - there some researchers might want to use the natural correlations in the data, but luckily that is an argument you can largely sidestep. 

Point 2
I suspect the most ardent believer in algorithmic bias will want some paragraph in intro that gives some ground on disparate impact versus treatment. One way you could do that without undermining the content of what you are doing is to cede a bit of ground where you describe the ideal experiments: 
* Disparate treatment: Manipulate protected characteristics
* Disparate impact: Manipulate characteristics that *in the world* for applications of interest covary highly with the protected characteristic

Your technique allows you to do both but highlights the need when doing disparate impact of needing the imagined covariances in the data (what X in the world in this application are you asserting varies with race?) rather than using whatever spurious correlation occurs in convenience samples. So what's nice is that you make both disparate impact and disparate treatment "causal" and requiring manipulation. The only distinction is what is being manipulated. 

Sendhil

\section{Comments from Kearns - 2020-05-13}
Hey Pietro — so I had a read of your paper. It’s a very compelling and interesting
piece of work, and very well-written as well; I understood most all of it even though
I am not in vision.

I think my main expository comment would be that in the main body of your paper,
the take-away message for non-vision people kind of gets a bit sublimated due to
the long and careful discussion of methodology. E.g. If I take the last sentence of
your abstract:

We validate our method by comparing it with the traditional observational method in ana-lyzing bias in gender classification algorithms. The two methods reach starkly different con-clusions. While the observational method detects gender and skin color bias, the experimentalmethod reveals bias due to hairstyle, and age

…I think it might help expand the audience for your paper if you discussed this last sentence
in much greater detail right up front in the paper. For a non vision/technical person, this takeaway
about the nature of bias and the two methods is perhaps the top-level message so might warrant
more and earlier discussion.

In terms of citations — in addition to my book with Aaron, in the places you discuss fairness
wrt intersectionality and combinations of features, you might want to cite these more technical
works on the topic:

Preventing Fairness Gerrymandering: Auditing and Learning for Subgroup Fairness. M.Kearns, S. Neel, A. Roth, and S. Wu. ICML 2018. https://arxiv.org/abs/1711.05144

An Empirical Study of Rich Subgroup Fairness for Machine Learning. M. Kearns, S. Neel, A. Roth, and S. Wu. ACM FAT* 2019. https://arxiv.org/abs/1808.08166

Ursula H ´ebert-Johnson, Michael P Kim, Omer Reingold, and Guy N Rothblum. Calibration for the (computationally-identifiable) masses. arXiv preprint arXiv:1711.08513, 2017.

Congratulations on an excellent work and talk soon!

Best
Michael


==> method.tex <==
\section{Method}
\label{sec:causal-analysis}

Our framework consists of two components: a technique to synthesize sets of images with control over semantic attributes, and a procedure using these synthesized images, along with human annotators, to perform analysis of a recognition system. 

In Section~\ref{sec:transect} we present a technique for attribute-controlled image synthesis. We introduce the \emph{transect}, a grid-like construct of synthesized images with a different attribute manipulated along each axis. A transect gives control over the joint distribution of synthesized attributes, unlike related methods that operate on a single attribute at a time~\cite{denton2019detecting,shen2019interpreting}. We then collect human annotations for each transect image, to precisely quantify our modifications.

In Section~\ref{sec:analysis} we present analyses we can perform using the annotated transects. We report a classifier's error rate, stratified along subroups of a sensitive attribute. We also return a covariate-adjusted estimate of the \emph{average causal effect} of a binary attribute on the classifier's performance. 

\subsection{Transects: A Walk in Face Space}
\label{sec:transect}
We assume a black-box face generator $G$ that can transform a latent vector $\bz \in \mathcal{R}^D$ into an image $I = G(\bz)$, where $p(\bz)$ is a distribution we can sample from. In our study, $G$ is the generator of a trained state-of-the-art GAN~\cite{karras2019style,karras2019analyzing}. GAN latent spaces typically exhibit good disentanglement of semantic image attributes. In particular, empirical studies show that each image attribute often has a direction $\bv \in \mathcal{R}^D$ that predominantly captures its variability~\cite{karras2019style,zhou2018interpreting}. We base our approach on a recent study~\cite{zhou2018interpreting} for single attribute traversals in GAN latent spaces. That method trains a linear model to predict a particular image attribute from $\bz$, and uses the model to traverse the $\bz$-space in a discriminative direction. Our method builds on this to synthesize image grids, i.e. \emph{transects}, spanning arbitrarily many attributes.  

\begin{figure}[t!]
\begin{center}
\includegraphics[width=\textwidth]{figures/single-transects.pdf}
\end{center}
\vspace{-0.3in}
\caption{{\bf 1D transects.} $1\times 5$ sample transects synthesized by our method for various attributes.}
\label{fig:single-transect-examples}
\end{figure}

\begin{figure}[t!]
\begin{center}
\includegraphics[width=\textwidth]{figures/multi-transects.pdf}
\end{center}
\vspace{-0.3in}
\caption{{\bf 2D transects.} Examples of $5 \times 5$ transects varying hair length and skin tone. Multidimensional transects allow for analysis across the joint distribution of multiple attributes. }
\label{fig:multi-transect-examples}
%\commentGB{These are pixelated, replace with high-res.}
\end{figure}

\subsubsection{Estimating Latents-to-Attributes Linear Models.}
\label{sec:latent-classifier}
We first sample the latent space, measure the attributes at each location through human observers, and use these measurements to impose an attribute coordinate system on the face space. More formally, let $A = \{a_1, \cdots, a_d\}$ be a set of $d$ image attributes (age, gender, skin color etc.).  We generate an annotated training dataset $\mathcal{D}=\{\bz^i, \by^i\}_{i=1}^N$, where $\by^i_j$ is a label for attribute $a_j$ for generated image $G(\bz^i)$. $\by^i_j$ may be continuous in $[0, 1]$ or binary in $\{0, 1\}$, depending on the nature of attribute $a_j$. 

We sample values of $\bz^i$ from $p(\bz)$ and obtain labels through human annotators. A related study obtains labels by only processing the generated images through a trained classifier~\cite{zhou2018interpreting}. We generally avoid this approach because any biases of the classifier due to attribute correlations --- precisely the phenomena we are trying to avoid --- will leak into our method. %However, some attributes may not be well-represented in the limited samples we collect. In these cases, we do use a trained classifier to label additional samples. 

For each attribute $a_j$ we use $\mathcal{D}$ to compute a $(D-1)$-dimensional linear hyperplane $h_j = (\bn_j, b_j)$, where $\bn_j$ is the normal vector and $b_j$ is the offset. For continuous attributes like age or skin color, we train a ridge regression model~\cite{hoerl1970ridge}. For binary attributes like ``has eyeglasses'' we train a support vector machine (SVM) classifier~\cite{cortes1995support}. 

\subsubsection{Multi-attribute Transect Generation.} The face space coordinate system may now be used to sample faces that vary along specific attributes. More formally: 
the hyperplane $h_j$ specifies the subspace of $\mathcal{R}^D$ with boundary or neutral values of attribute $a_j$, and the normal vector $\bn_j$ specifies a direction along which $a_j$ primarily varies. To construct a one-dimensional, length-$L$ transect for $a_j$, we start with a random point $\bz^i$, project this point onto $h_j$, and query $L-1$ total points from both sides of the boundary along $\bn_j$. Fig.~\ref{fig:single-transect-examples} presents some single transect examples. 

We generalize to $K$-dimensional transects in Algorithm~\ref{alg:multi}. The main extensions are: (1) we project $\bz^i$ onto the intersection of $K$ attribute hyperplanes, and (2) we move in a $K$-dimensional grid in $\bz$-space (see Fig.~\ref{fig:multi-transect-examples}). Input $\bc$ stores grid distances from the hyperplane, and $\bv$ stores direction vectors (equivalent to $\bn$ here, until orthogonalization is introduced in the next section).

We are unaware of a simple closed-form solution to project $\bz^i$ onto the intersection of arbitrarily many hyperplanes. We instead take an iterative approach: we sequentially project the point onto each hyperplane, and repeat this process for some number of iterations. Repeated projections onto convex sets is guaranteed to converge to a location on the intersection of the sets~\cite{youla1987mathematical}. If the hyperplanes are perfectly orthogonal, this process converges in exactly one iteration; we empirically found convergence in less than 50 iterations. 

\begin{algorithm}[t!]
\textbf{Input}: Generator $G$, $K$ tuples $\{ (L_k, h_k, \bv_k, \bc_k) \}_{k=1}^K$, where $L_k$ is a transect dimension, $h_k$ is a hyperplane, $\bv_k$ is a direction vector, and $\bc_k$ are grid distances.\\
\textbf{Output}: A $L_1 \times \cdots \times L_K$ transect $T^i$. \\ 
\texttt{\\}
 $\bz^i \sim p(\bz)$\\
 $\bz^{i,0} = $ projection of $\bz^i$ onto intersection of $\{h_k\}_{k=1}^K$\\
 \For{$l_1=1 \cdots L_1$}{
    $\vdots$\\
    \For{$l_K=1 \cdots L_K$}{
    $T^i(l_1, \cdots , l_K) = G( \bz^{i,0} + \sum_{k=1}^K \bc_k[l_k] \cdot \bv_k)$\;
    }
 }
 \caption{$K$-attribute Transect Generation}
 \label{alg:multi}
\end{algorithm}
\subsubsection{Orthogonalization of Traversal Directions}
The hyperplane normals $\{\bn_j\}_{j=1}^{d}$ are not orthogonal to one another. If they are used as traversal directions, we may observe unwanted coupling of attribute modifications. We mitigate this effect by producing a set of direction vectors $\{\tilde{\bn}_j\}_{j=1}^d$, where $\tilde{\bn}_j \perp \bn_k, \forall k \neq j$. Details on the orthogonalization procedure are in supplementary material. We also modify the grid locations $\bc_j$ to account for this change: $\tilde{\bc}_j = \frac{\bc_j}{\langle \bn_j, \tilde{\bn}_j \rangle}$, and feed $\tilde{\bn}$ and $\tilde{\bc}$ as direction vectors and grid distances into Algorithm~\ref{alg:multi}.

\subsubsection{Setting Step Sizes and Transect Dimensions}
\label{sec:step-sizes}
If human annotation cost were negligible, we could simply query many grid locations with a large transect dimension $L$ to capture subtle appearance changes over the dynamic ranges of the attributes. But given constrained resources, we set $L$ to a small value, e.g., $L=5$. For each attribute, we manually set minimum and maximum signed distances to its hyperplane, and linearly interpolate $L$ points between these extremes. We set per-attribute min/max distances so that the resulting transects depict a full dynamic range for most random samples.

\subsection{Analyses Using Transects}
\label{sec:analysis}
Transects sometimes alter more than just their intended attributes. The degree to which an attribute is altered is also not uniform across transects. To account for these factors, we collect a second set of human annotations --- identical in design to those collected in Section~\ref{sec:latent-classifier} --- yielding a dataset of transect images with labels. We perform two types of analyses on gender classifier $C$ with this dataset, for a binary attribute of interest $s \in \{0, 1\}$. 

We would like to estimate the mean difference in the \emph{potential} error of $C$ when $s=1$ versus $s=0$ for each image. The word `potential' delineates a counterfactual outcome that we do not have access to, from an observed outcome in our dataset. Such a measure is traditionally known as the ``average treatment effect"(ATE) of $s$. Estimating ATE from observational data is a well-studied, fundamental task in causal inference~\cite{angrist1995identification,heckman2001instrumental,oreopoulos2006estimating,rubin2006matched}.

Our first analysis technique is the common strategy of reporting $C$'s error rate across subgroups stratified by $s$. Let $y^i$ be the true gender and $\hat{y}^i $ be $C$'s prediction for example $i$. Let $e^i = \ell (\hat{y}^i, y^i)$ be the classification error, where $\ell(\cdot, \cdot)$ is a loss function. We compute $E_1$ (and similarly, $E_0$), the average error of $C$ over test samples where $s^i=1$ ($s^i = 0$): 
\small
\begin{align}
E_1 = \frac{\sum_i e^i \mathbbm{1} (s^i = 1)}{ \sum_i \mathbbm{1} (s^i = 1)},
\end{align}
\normalsize
\noindent  We can also stratify across more than one attribute to focus on more refined subpopulations. If the two subgroups only vary by $s$, then $E_1 - E_0$ captures the true ATE. This is known in statistics as a \emph{matched study}. Our transects are generated in a way to better facilitate such studies than data ``from-the-wild" (see Sec.~\ref{sec:real-comparison} for empirical validation), but still can not perfectly achieve this gold-standard. A simple approach to estimate ATE while adjusting for covariates is to train a linear model predicting $e^i$ from $s$ and all other relevant covariates:
\small
\begin{align}
    e^i = \beta_0 + \beta_s s^i + \sum_{j=1}^{d-1}\beta_j x^i_j + \epsilon^i,
\end{align}
\normalsize
where $x$ are covariates, $\beta$s are coefficients, and $\epsilon$ is a noise term. $\beta_s$ captures the ATE~\cite{gelman2006data}, the average change in $e^i$ given one unit change in $s$, holding all other variables constant, provided: (1) a linear model is an appropriate choice to capture the relationship between the dependent and independent variables, (2) all relevant attributes are included in the model (i.e., no hidden confounders), and (3) no attributes that are affected by $s$ are included in the model, otherwise the model can explain away the impact of $s$ by using these factors instead. 

We can never be completely sure we have satisfied these conditions with observational data, especially with complex natural images. But by aiming for these standards, we take steps towards more causal analysis. Two notes about condition (1): continuous covariates will often not have a linear relationship with the outcome. A common remedy is to discretize these variables, and re-represent them with one-hot encodings~\cite{gelman2006data}. Finally, when the outcome lies in $[0, 1]$, as is the case with $e^i$, we use logistic instead of linear regression. $\beta_s$ then represents the expected change in the \emph{log odds} of $e^i$ for a unit change in $s$.

%Assuming that a linear model is appropriate, and that the appropriate variables are included (i.e., no confounder variables are missing, and no variables affected by $s$ are included), $\beta_s$ captures the ATE~\cite{gelman2006data}, the average change in $e^i$ given one unit change in $s$, holding all other variables constant. When the outcome variable is in $[0, 1]$ as is the case with $e^i$, we use a logistic regression model, and $\beta_s$ then represents the expected change in \emph{log odds} of $e^i$ for a unit change in $s$. In general, continuous covariates are not necessarily linearly related to the outcome variable. A common remedy is to discretize these variables, and re-represent them with one-hot encodings~\cite{gelman2006data}. 

\begin{comment}
\subsubsection{Boundary Shift Bias}
We now introduce a second, more fine-grained bias measure relating an attribute's effect on an analysis system's output. This measure is only meaningful for 
continuous attributes which we expect to have a monotonic relationship with the classifier's response function. An example is the relationship between hair length and gender estimation. 

For each transect, we are interested in finding the value of the continuous attribute where the system ``flips'' its decision on gender. We will then compare this value to the corresponding value of a `ground truth' decision system (the human annotators in our experiments), and report an average shift over many examples. Unlike bulk bias, this shift tells us precisely how much more (or less) of the attribute is needed to produce classification errors. 

We make use of the \emph{psychometric function} $\psi(x)$, used in psychoanalysis to quantify the relationship between a stimulus $x$ and the probability of a positive system response ~\cite{treutwein1999fitting,wichmann2001psychometric}. This function often takes the form:

\begin{align}
    \label{eqn:psychometric}
    \psi(x; \alpha, \beta, \gamma, \lambda) = \gamma + (1-\gamma - \lambda)F(x; \alpha, \beta), 
\end{align}
\noindent with $F(x)$ modeled by the logistic function:
\begin{align}
F(x; \alpha, \beta) = \frac{1}{1+e^{-4\beta\left(x-\alpha\right)}}.
\end{align}
The parameters $\alpha$ and $\beta$ specify the shift and slope of the logistic curve, and $\gamma$ and $\lambda$ specify the output range.

Given a $1\times L$ transect depicting modifications to a continuous attribute, we fit a ground truth function $\psi(x)$ to the set of $L$ point pairs, $\{x^i, y^i\}_{i=1}^{L}$, where $x^i$ is the attribute value, and $y^i$ is the annotators' gender score. We also fit a function, $\hat{\psi}(x)$, to the classification system's gender predictions. Our proposed boundary shift bias measure is simply the relative shift between the two curves: $\hat{\alpha} - \alpha$. Fig.~\ref{fig:psychometric} illustrates a psychometric function fit to a $1\times 13$ transect varying hair length.  

\begin{figure}[t!]
\begin{center}
\includegraphics[scale=0.25]{figures/mock-shift-bias-figure.pdf}
\end{center}
\commentPP{The figure is a mockup. The caption should be adjusted once we have the real figure.}
\commentGB{Pietro, this figure isn't exactly accurate, but maybe its fine for the Amazon review. In this image, we are fitting a curve from transect image number [-6, 6] to gender. It should really be between the hair length value of each image to gender.}
\caption{{\bf Measuring shift bias.} (Top) A transect of face images where one parameter (hair length) is systematically varied. (Bottom) Measurements from two systems being tested (red and green dots) and from human annotators (blue). Psychometric curves (sigmoids) are fit to each set of measurement points. The inflection of each psychometric curve is the nominal place where the transition takes place. The {\em shift bias} of each system is measured as the difference between that system's transition coordinate and the human annotators' transition coordinate.}
\label{fig:shift-bias}
\end{figure}

Let $g(\cdot): \mathcal{R}^{W\times H \times 3} \rightarrow \mathcal{R}$ be a function returning the average annotator gender score for an input image, and let $\hat{g}(\cdot): \mathcal{R}^{W\times H \times 3} \rightarrow \mathcal{R}$ return the classifier's gender score. 
\end{comment}
